Auroras on Mars: from Discovery to New Developments

Auroras are emissions in a planetary atmosphere caused by its interactions with the surrounding plasma environment. They have been observed in most planets and some moons of the solar system. Since their first discovery in 2005, Mars auroras have been studied extensively and is now a rapidly growing area of research. Since Mars lacks an intrinsic global magnetic field, its crustal field is distributed throughout the planet and its interactions with the surrounding plasma environment lead to a number of complex processes resulting in several types of auroras uncommon on Earth. Martian auroras have been classified as diffuse, discrete and proton aurora. With new capability of synoptic observations made possible with the Hope probe, two new types of auroras have been observed. One of them, which occurs on a much larger spatial scale, covering much of the disk, is known as discrete sinuous aurora. The other subcategory is one of proton auroras observed in patches. Further study of these phenomena will provide insights into the interactions between the atmosphere, magnetosphere and the surrounding plasma environment of Mars. We provide a brief review of the work done on the subject in the past 17 years since their discovery, and report new developments based on observations with Hope probe.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


